What Makes a Scientific Paper be Accepted for Publication?

Despite peer-reviewing being an essential component of academia since the 1600s, it has repeatedly received criticisms for lack of transparency and consistency. We posit that recent work in machine learning and explainable AI provide tools that enable insights into the decisions from a given peer review process. We start by extracting global explanations in the form of linguistic features that affect the acceptance of a scientific paper for publication on an open peer-review dataset. Second, since such global explanations do not justify causal interpretations, we provide a methodology for detecting confounding effects in natural language in order to generate causal explanations, under assumptions, in the form of lexicons. Our proposed linguistic explanation methodology indicates the following on a case dataset of ICLR submissions: a) the organising committee follows, for the most part, the recommendations of reviewers, and, b) the paper's main characteristics that led to reviewers recommending acceptance for publication are originality, clarity and substance.

==> tab/auc_lr_curves.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Classification Task }                    & \textbf{Model} & \multicolumn{1}{c}{\textbf{AUC}} \\ \hline
\multirow{2}{*}{Meta-Reviews}           & GRU+ATTN  & \textbf{39.84}           \\
                                        & BERT+LIME & 33.61                    \\ \hline
\multirow{2}{*}{Individual Peer Review} & GRU+ATTN  & 28.39                    \\
                                        & BERT+LIME & \textbf{31.13}           \\ \hline
Final Decision Peer Review              & BERT+LIME & \textbf{32.62}           \\ \hline
\end{tabular}
\caption{AUC (Area Under Curve) of the Logistic Regression curves for the different classifiers.}
\label{tab:auc_lr}
\end{table*}

==> tab/meta_expl_tab_residual.tex <==
\begin{table*}[h!]
\centering
{\fontsize{12pt}{12pt}\selectfont
\begin{tabular}{ll}
\hline
\textbf{GRU (Non-Causal)}     &\textbf{ GRU (DR+ATTN) }\\ \hline
positively       & nicely          \\
accept           & overcomplicated \\
suspiciously     & positively      \\
wrong            & yet             \\
yet              & rebuttal        \\
perhaps          & ready           \\
mix              & sufficiently    \\
limit            & properly        \\
guidance         & acceptance      \\
read             & surprise        \\
impressive       & usual           \\
surprise         & into            \\
enough           & describe        \\
incremental      & finding         \\
sufficiently     & organize        \\
timely           & execution       \\
journal          & insight         \\
post             & receive         \\
contribute       & criterion       \\
ready            & overall         \\
not              & good            \\
variational      & closely         \\
nicely           & wise            \\
receive          & suspiciously    \\
submit           & well            \\
relevant         & badly           \\
much             & write           \\
high             & pair            \\
weak             & explain         \\
good             & not             \\
write            & simple          \\
whilst           & weak            \\
into             & asset           \\
below            & great           \\
benefit          & out             \\
rebuttal         & execute         \\
generative       & helpful         \\
strengthen       & enjoy           \\
meet             & conditional     \\
variety          & mix             \\
give             & entirely        \\
hide             & contribution    \\
recommend        & world           \\
badly            & demonstrate     \\
long             & accept          \\
clear            & assume          \\
convince         & post            \\
gain             & publication     \\
serious          & effective       \\
maintain         & clearly         \\ \hline
\end{tabular}
\caption{Top 50 salient words for meta-reviews. The first column contains the explanations of the non-causal models. The second column contains the deconfounded lexicon.}
\label{tab:meta_exp_residual}
}
\end{table*}

==> tab/non_causal_explanations.tex <==
\begin{table*}[]
\centering
{\fontsize{12pt}{12pt}\selectfont
\begin{tabular}{lllll}
\hline
\begin{tabular}[c]{@{}l@{}}\textbf{BERT -}\\ \textbf{Meta-Review}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{GRU -}\\ \textbf{Meta-Review}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{BERT -}\\ \textbf{Individual}\\ \textbf{Peer Review}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{GRU -}\\\textbf{ Individual}\\\textbf{ Peer Review}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{BERT -}\\ \textbf{Final Decision}\\\textbf{ Peer Review}\end{tabular} \\ \hline
enjoyed                                                     & positively                                                 & interspeech                                                            & not                                                                   & kolter                                                                     \\
cnns                                                        & accept                                                     & zhang                                                                  & attempt                                                               & aaai                                                                       \\
resubmit                                                    & suspiciously                                               & prons                                                                  & comprehensive                                                         & not                                                                        \\
community                                                   & wrong                                                      & dismissed                                                              & interfere                                                             & third                                                                      \\
limited                                                     & yet                                                        & third                                                                  & variational                                                           & efficiently                                                                \\
experimentation                                             & perhaps                                                    & p6                                                                     & entirely                                                              & untrue                                                                     \\
3                                                           & mix                                                        & confusing                                                              & systematically                                                        & cifar10                                                                    \\
workshop                                                    & limit                                                      & resulting                                                              & perfect                                                               & venue                                                                      \\
poster                                                      & guidance                                                   & geometry                                                               & sure                                                                  & recovered                                                                  \\
topic                                                       & read                                                       & unconvincing                                                           & lda                                                                   & huffman                                                                    \\
variational                                                 & impressive                                                 & honestly                                                               & formalize                                                             & riemannian                                                                 \\
limit                                                       & surprise                                                   & not                                                                    & tolerant                                                              & cifar                                                                      \\
although                                                    & enough                                                     & community                                                              & valid                                                                 & arxiv                                                                      \\
not                                                         & incremental                                                & cannot                                                                 & belief                                                                & accompanying                                                               \\
sound                                                       & sufficiently                                               & superficial                                                            & gan                                                                   & extended                                                                   \\
none                                                        & timely                                                     & readership                                                             & imposible                                                             & convex                                                                     \\
accepted                                                    & journal                                                    & big                                                                    & adagrad                                                               & github                                                                     \\
dropout                                                     & post                                                       & suggestion                                                             & semantically                                                          & trace                                                                      \\
imagenet                                                    & contribute                                                 & dialogue                                                               & aware                                                                 & eigenspectra                                                               \\
agent                                                       & ready                                                      & revisit                                                                & clear                                                                 & encourage                                                                  \\
justify                                                     & not                                                        & bag                                                                    & carefully                                                             & code                                                                       \\
generative                                                  & variational                                                & analysed                                                               & j.                                                                    & asynchronous                                                               \\
advantage                                                   & nicely                                                     & icml                                                                   & and/or                                                                & crucial                                                                    \\
unfortunately                                               & receive                                                    & taken                                                                  & arguably                                                              & auxiliary                                                                  \\
video                                                       & submit                                                     & typo                                                                   & fully                                                                 & investigated                                                               \\
review                                                      & relevant                                                   & submitted                                                              & offer                                                                 & iclrw2016                                                                  \\
solver                                                      & much                                                       & energy                                                                 & vs.                                                                   & hyperparameters                                                            \\
three                                                       & high                                                       & nice                                                                   & confident                                                             & discus                                                                     \\
task                                                        & weak                                                       & spirit                                                                 & message                                                               & dcgan                                                                      \\
use                                                         & good                                                       & competitive                                                            & object                                                                & interesting                                                                \\
confident                                                   & write                                                      & per                                                                    & receive                                                               & nice                                                                       \\
generalisation                                              & whilst                                                     & highlighted                                                            & probably                                                              & game                                                                       \\
supervised                                                  & into                                                       & multimodality                                                          & multimodality                                                         & demonstration                                                              \\
promise                                                     & below                                                      & far                                                                    & strictly                                                              & lample                                                                     \\
raised                                                      & benefit                                                    & 04562                                                                  & directly                                                              & the                                                                        \\
understanding                                               & rebuttal                                                   & lack                                                                   & twitter                                                               & significance                                                               \\
timely                                                      & generative                                                 & preprint                                                               & join                                                                  & seq2seq                                                                    \\
reject                                                      & strengthen                                                 & dcgan                                                                  & e.g.                                                                  & community                                                                  \\
unsatisfactory                                              & meet                                                       & conduct                                                                & observe                                                               & perspective                                                                \\
yet                                                         & variety                                                    & word2vec                                                               & complete                                                              & paper                                                                      \\
mixed                                                       & give                                                       & wen                                                                    & explain                                                               & thanks                                                                     \\
shot                                                        & hide                                                       & gan                                                                    & novelty                                                               & investigates                                                               \\
propose                                                     & recommend                                                  & rejected                                                               & dualnets                                                              & insightful                                                                 \\
how                                                         & badly                                                      & start                                                                  & convince                                                              & uploaded                                                                   \\
rejection                                                   & long                                                       & towards                                                                & handle                                                                & narrow                                                                     \\
thus                                                        & clear                                                      & multiplication                                                         & nintendo                                                              & match                                                                      \\
salimans                                                    & convince                                                   & generalisation                                                         & theorem                                                               & seed                                                                       \\
provided                                                    & gain                                                       & auxiliary                                                              & satisfy                                                               & tsp                                                                        \\
goal                                                        & serious                                                    & parametric                                                             & ready                                                                 & adversarial                                                                \\
reservation                                                 & maintain                                                   & enjoyed                                                                & demand                                                                & isn                                                                        \\ \hline
\end{tabular}
\caption{Top 50 salient words for non-causal models.}
\label{tab:peer_expl}
}
\end{table*}

==> tab/peer_expl_bow_tab_residual.tex <==
\begin{table*}[h!]
\centering
{\fontsize{12pt}{12pt}\selectfont
\begin{tabular}{ll}
\hline
\textbf{BoW (Non-Causal)  }              & \textbf{BoW (DR+BoW)  }                  \\ \hline
(not, enough)                & (not, enough)                \\
(much, be)                   & (much, be)                   \\
(literature, and)            & (not, compare)               \\
(need, a)                    & (evidence, to)               \\
(evidence, to)               & (be, insufficient)           \\
(be, not, enough)            & (comparison, with, other)    \\
(not, compare)               & (be, mention)                \\
(on, use)                    & (literature, and)            \\
(comparison, with, other)    & (need, a)                    \\
(doe, not, provide)          & complementary                \\
(claim, that, this)          & (be, not, enough)            \\
(network, weight)            & (method, need)               \\
(do, not, compare)           & (would, require)             \\
(work, need)                 & (doe, not, provide)          \\
gans                         & (on, use)                    \\
(layer, this)                & (to, compare, the)           \\
(be, insufficient)           & (have, see)                  \\
(it, look, like)             & (comparison, with, the)      \\
(push, the)                  & (network, weight)            \\
(work, so)                   & (do, not, compare)           \\
(to, compare, the)           & (sure, if, the)              \\
(not, compare, to)           & (no, quantitative)           \\
(not, surprise)              & (no, new)                    \\
(and, compare, to)           & (experiment, there, be)      \\
(have, see)                  & (on, the, previous)          \\
(very, hard)                 & (improve, version)           \\
(of, the, dataset)           & (not, compare, to)           \\
(be, mention)                & (adversarial, train, to)     \\
(should, be, mention)        & (dataset, which, be)         \\
(not, find, the)             & (limit, in)                  \\
(not, ready)                 & (experiment, there)          \\
(novelty, and)               & (layer, this)                \\
(no, quantitative)           & (work, so)                   \\
(the, theoretical, analysis) & (be, write)                  \\
(experiment, there)          & (the, basis)                 \\
(no, new)                    & (claim, that, this)          \\
(to, control)                & (not, ready)                 \\
complementary                & (work, need)                 \\
(would, require)             & (the, theoretical, analysis) \\
(enough, detail)             & incomplete                   \\
(train, neural, network)     & (reasonably, good)           \\
(of, video)                  & (it, hard, to)               \\
(the, combination, of)       & (a, system)                  \\
incomplete                   & (and, compare, to)           \\
(the, claim, about)          & gans                         \\
(they, introduce)            & (they, introduce)            \\
(comparison, on)             & (result, be, provide)        \\
(limit, in)                  & (not, find, the)             \\
push                         & (should, be, mention)        \\
(cover, a)                   & (push, the)                  \\ \hline
\end{tabular}
\caption{Top 50 salient n-grams for peer reviews and top 50 deconfounded n-grams.}
\label{tab:peer_expl_bow_residual}
}
\end{table*}

==> tab/peer_expl_tab_residual.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[h!]
\centering
{\fontsize{12pt}{12pt}\selectfont
\begin{tabular}{llll}
\hline
\textbf{BERT (Non-Causal)}    & \textbf{BERT (DR+LIME) }& \textbf{GRU (Non-Causal)} &\textbf{ GRU (DR+ATTN) }\\ \hline
interspeech       & interspeech    & not              & identical      \\
zhang             & dismissed      & attempt          & sure           \\
prons             & prons          & comprehensive    & premise        \\
dismissed         & geometry       & interfere        & carefully      \\
third             & p6             & variational      & heavy          \\
p6                & submitted      & entirely         & specify        \\
confusing         & unfair         & systematically   & tease          \\
resulting         & unconvincing   & perfect          & interfere      \\
geometry          & readership     & sure             & necessarily    \\
unconvincing      & honestly       & lda              & adagrad        \\
honestly          & not            & formalize        & attempt        \\
not               & spirit         & tolerant         & novelty        \\
community         & confusing      & valid            & fully          \\
cannot            & analysed       & belief           & repeat         \\
superficial       & bag            & gan              & systematically \\
readership        & unable         & imposible        & not            \\
big               & cannot         & adagrad          & gray           \\
suggestion        & rejected       & semantically     & theoretically  \\
dialogue          & insightful     & aware            & anymore        \\
revisit           & multiplication & clear            & role           \\
bag               & highlighted    & carefully        & belief         \\
analysed          & enjoyed        & j.               & recommendation \\
icml              & misleading     & and/or           & almost         \\
taken             & disagree       & arguably         & consistently   \\
typo              & dialogue       & fully            & primary        \\
submitted         & mu\_           & offer            & subtraction    \\
energy            & wen            & vs.              & good           \\
nice              & lack           & confident        & satisfactory   \\
spirit            & nice           & message          & background     \\
competitive       & multimodality  & object           & write          \\
per               & welcome        & receive          & compute        \\
highlighted       & conduct        & probably         & easy           \\
multimodality     & recommender    & multimodality    & teach          \\
far               & encourage      & strictly         & enough         \\
04562             & dualnets       & directly         & convince       \\
lack              & thanks         & twitter          & except         \\
preprint          & cdl            & join             & ready          \\
dcgan             & preprint       & e.g.             & explain        \\
conduct           & 04562          & observe          & usage          \\
word2vec          & enjoy          & complete         & sell           \\
wen               & revisit        & explain          & unfortunately  \\
gan               & community      & novelty          & arguably       \\
rejected          & appreciate     & dualnets         & yet            \\
start             & principled     & convince         & especially     \\
towards           & medical        & handle           & elegantly      \\
multiplication    & coding         & nintendo         & sufficiently   \\
generalisation    & drnn           & theorem          & handle         \\
auxiliary         & accompanying   & satisfy          & cdl            \\
parametric        & factorization  & ready            & setup          \\
enjoyed           & jmlr           & demand           & resception     \\ \hline
\end{tabular}
\caption{Top 50 salient words for the task of Individual Peer Classification. In order to make comparisons, we present both causal and non-causal models.}
\label{tab:peer_expl_residual}
}
\end{table*}

==> tab/top50_tab.tex <==
\begin{table*}[h!]
\centering
{\fontsize{9pt}{9pt}\selectfont
\begin{tabular}{llll}
\hline
\textbf{SciBERT (Non-Causal)}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & \textbf{SciBERT (DR+LIME)}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \textbf{GRU (Non-Causal)}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & \textbf{GRU (DR+ATTN)}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\begin{tabular}[c]{@{}l@{}}interspeech, zhang, prons,\\ dismissed, third, p6, \\ confusing, resulting, \\ geometry, unconvincing, \\ honestly, not,community, \\ cannot, superficial,\\ readership, big, suggestion, \\ dialogue, revisit, bag, \\ analysed, icml, taken, typo, \\ submitted, energy, nice, \\ spirit, competitive, per,\\ highlighted, multimodality, \\ far, 04562, lack, preprint, \\ dcgan, conduct, word2vec,\\ wen, gan, rejected, start, \\ towards, multiplication,\\ generalisation, auxiliary, \\ parametric, enjoyed\end{tabular} & \begin{tabular}[c]{@{}l@{}}interspeech, dismissed, prons, \\ geometry, p6, submitted,\\ unfair, unconvincing,\\ readership, honestly, not, \\ spirit, confusing, analysed, \\ bag, unable, cannot, rejected, \\ insightful, multiplication,\\ highlighted, enjoyed, \\ misleading, disagree, \\ dialogue,mu\_, wen, lack, \\ nice, multimodality, welcome, \\ conduct, recommender, \\ encourage, dualnets, thanks,\\ cdl, preprint, 04562, enjoy,\\ revisit, community, appreciate, \\ principled, medical, coding, \\ drnn, accompanying, \\ factorization, jmlr\end{tabular} & \begin{tabular}[c]{@{}l@{}}not, attempt,\\ comprehensive, interfere, \\ variational, entirely, \\ systematically, perfect,\\ sure, lda, formalize, \\ tolerant, valid, belief, gan, \\ imposible, adagrad, \\ semantically, aware, clear, \\ carefully, j., and/or, \\ arguably, fully, offer, vs., \\ confident, message, object, \\ receive, probably, \\ multimodality, strictly, \\ directly, twitter, join, e.g., \\ observe, complete, explain, \\ novelty, dualnets, convince, \\ handle, nintendo, theorem, \\ satisfy, ready, demand\end{tabular} & \begin{tabular}[c]{@{}l@{}}identical, sure, premise,\\ carefully, heavy, specify,\\ tease, interfere, necessarily, \\ adagrad, attempt, novelty, \\ fully, repeat, systematically, \\ not, gray, theoretically,\\ anymore, role, belief, \\ recommendation, almost,\\ consistently, primary, \\ subtraction, good, \\ satisfactory, background, \\ write, compute, easy, teach, \\ enough, convince, except,\\ ready, explain, usage, sell,\\ unfortunately, arguably, \\ yet, especially, elegantly, \\ sufficiently, handle,\\ cdl, setup, reception\end{tabular} \\ \hline
\end{tabular}
\caption{Top 50 salient words for Individual Peer Review Classification. We present class-agnostic explanations both for some of the non-causal models (Section \ref{sec:data_expl}) and for some DR models (Section \ref{sec:causal}).
}
\label{tab:top50}
}
\end{table*}

==> tab/top5_tab.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
{\fontsize{10pt}{10pt}\selectfont
\begin{tabular}{llll}
\hline
\textbf{SciBERT (Non-Causal)}    & \textbf{SciBERT (DR+LIME) }& \textbf{GRU (Non-Causal)} &\textbf{ GRU (DR+ATTN) }\\ \hline
interspeech  & interspeech    & not            & identical      \\
zhang        & dismissed      & attempt        & sure           \\
prons        & prons          & comprehensive  & premise        \\
dismissed    & geometry       & interfere      & carefully      \\
third        & p6             & variational    & heavy          \\ 
p6                & submitted      & entirely         & specify        \\
confusing         & unfair         & systematically   & tease          \\
resulting         & unconvincing   & perfect          & interfere      \\
geometry          & readership     & sure             & necessarily    \\
unconvincing      & honestly       & lda              & adagrad        \\
\hline
\end{tabular}
\caption{Top 10 salient words for Individual Peer Review Classification. We present explanations both for some of the non-causal models (Section \ref{sec:data_expl}) and for some causal model (Section \ref{sec:causal}).
}
\label{tab:top5}
}
\end{table*}
